COLA: Consistent Learning with Opponent-Learning Awareness

Learning in general-sum games is unstable and frequently leads to socially undesirable (Pareto-dominated) outcomes. To mitigate this, Learning with Opponent-Learning Awareness (LOLA) introduced opponent shaping to this setting, by accounting for each agent's influence on their opponents' anticipated learning steps. However, the original LOLA formulation (and follow-up work) is inconsistent because LOLA models other agents as naive learners rather than LOLA agents. In previous work, this inconsistency was suggested as a cause of LOLA's failure to preserve stable fixed points (SFPs). First, we formalize consistency and show that higher-order LOLA (HOLA) solves LOLA's inconsistency problem if it converges. Second, we correct a claim made in the literature by Sch\"afer and Anandkumar (2019), proving that Competitive Gradient Descent (CGD) does not recover HOLA as a series expansion (and fails to solve the consistency problem). Third, we propose a new method called Consistent LOLA (COLA), which learns update functions that are consistent under mutual opponent shaping. It requires no more than second-order derivatives and learns consistent update functions even when HOLA fails to converge. However, we also prove that even consistent update functions do not preserve SFPs, contradicting the hypothesis that this shortcoming is caused by LOLA's inconsistency. Finally, in an empirical evaluation on a set of general-sum games, we find that COLA finds prosocial solutions and that it converges under a wider range of learning rates than HOLA and LOLA. We support the latter finding with a theoretical result for a simple game.

==> results_outline.tex <==
\section{Results}
\label{results}
% Results Section Introduction.
% First, we look at learning outcomes
% Second, compare update functions and consistency

We split the Results section into two parts. First, we qualitatively analyze COLA's learning outcomes, including an empirical investigation of our theoretical results (Propositions \ref{consistency_not_unique}, \ref{consistency_sfps}, and \ref{prop:hamiltonian_theory}) and a qualitative comparison to SOS, LOLA, and CGD to identify the benefits and effects of increased consistency. On the Tandem game, we show that CGD does not coincide with the learning outcome of higher-order LOLA, whereas COLA does.
Second, we compare the consistency losses of LOLA, HOLA, and COLA and investigate when iLOLA and COLA coincide. We analyze multiple look-ahead rates because we found that different look-ahead rates lead to different learning outcomes. For example, on the IPD, LOLA finds Defect-Defect at low look-ahead rates and Tit-for-Tat at higher look-ahead rates.
Additional results can be found in Appendix~\ref{appendix-further-results}.


\paragraph{Learning Outcomes.}
% We compare the learning behavior in the underlying games to other SOTA algorithms
We analyze the learning outcomes achieved by COLA update functions qualitatively and compare to those found by LOLA, HOLA, SOS and CGD. 

% In the Tandem game:
% We get results that confirm our consistency loss comparison
% We find that COLA does not recover SFPS
% COLA works at high look-ahead rates
In the Tandem game (Figure \ref{fig:tandem_play}), we can see that COLA and HOLA8 converge to similar outcomes in the game, whereas CGD does not.  Moreover, COLA does not recover SFPs, thus experimentally confirming Proposition~\ref{consistency_sfps}. In contrast to LOLA, HOLA and SOS, COLA finds a convergent solution even at a high look-ahead rate (see COLA:0.8), whereas  do not (Figure \ref{fig:tandem_play_div} in Appendix \ref{appendix:tandem}). CGD is the only other algorithm in the comparison that also shows robustness to high look-ahead rates in the Tandem game. 

% COLA works well with high look-ahead rates on MP
On Matching Pennies at high look-ahead rates, SOS and LOLA mostly don’t converge whereas COLA converges even faster with a high look-ahead rate (see Figure \ref{fig:var_cons_high}), confirming Proposition \ref{prop:hamiltonian_theory} experimentally.

% COLA finds fair solution consistently
For the Ultimatum game, the qualitative comparison shows that COLA is the only method that finds the fair solution consistently at a high look ahead rate, whereas SOS, LOLA, and CGD do not (see Figure \ref{fig:ult_cons_high} in Appendix \ref{appendix:ult}). At low look-ahead rates, all algorithms find the unfair solution (Figure \ref{fig:ult_play}).

% COLA finds fair solution on Chicken game
For further comparison, we introduce the Chicken game in Appendix \ref{appendix:chicken_game}. Both Taylor LOLA and SOS crash, whereas COLA swerves at high look-ahead rates (Figure \ref{fig:chicken_play_high}). Crashing in the Chicken game results in a catastrophic payout for both agents, whereas swerving results in a jointly preferable outcome. Interestingly, in contrast to Taylor LOLA, exact LOLA swerves. The Chicken game is the only game where we found a difference in learning behavior between exact LOLA and Taylor LOLA. 

% COLA finds something comparable to T4T on IPD
On the IPD, all algorithms find the Defect-Defect strategy on low look-ahead rates (Figure \ref{fig:ipd_play_low}). At high look-ahead rates, COLA finds a strategy qualitatively similar to Tit-for-Tat, as displayed in Figure \ref{fig:ipd_policy}, though much more noisy. However, COLA still achieves close to the optimal joint loss, in comparison to CGD, which finds Defect-Defect even at a high look-ahead rate (see Figure \ref{fig:cgd_on_ipd} in Appendix \ref{appendix:ipd}). 

% We show that variance of learning behaviour is reduced with increased consistency on the Matching Pennies game.
To further motivate the point that increased consistency helps with robustness to a wider range of look-ahead rates, we plot the consistency of update functions against the variance of losses during learning achieved by these update functions in the Matching Pennies game at a high look-ahead rate in Figure \ref{fig:mp_div}. The lower the consistency loss, the lower the variance of payoff trajectory. This further underlines, at least empirically, the benefits of increased consistency.

\paragraph{Update functions.}
Next, we continue with an in-depth analysis of the consistency losses. In general, we want to numerically investigate if and when COLA coincides with iLOLA. Furthermore, we are interested in the role of the look-ahead rate on the consistency loss, as the look-ahead rate influences, what learning outcome we observe.
%  HOLA consistency loss behaviour on a set of games
First, we investigate how increasing the order of HOLA affects the consistency of its updates. As we can see in Table \ref{tab:beta_hola}, \ref{tab:imp_cons} and \ref{tab:ipdcons}, HOLA's updates become more consistent with increasing order, but only below a certain look-ahead rate threshold. Above that threshold, HOLA's updates become less consistent with increasing order. The threshold is game-specific. In the Tandem game, it is around a look-ahead rate of 0.5, for the IPD around 0.1 and MP around 0.5. 
Such a threshold can be found empirically for all games that we evaluate on, as we show in Appendix~\ref{appendix-further-results} in Tables \ref{tab:ham_cons}, \ref{tab:bal_cons}, \ref{tab:ult_cons} and \ref{tab:chicken_cons}.

% Compare COLA and HOLA consistency losses
Second, we compare the consistency losses of COLA and HOLA. In the aforementioned Tables, we observe that COLA achieves low consistency losses on most games. Below the threshold, COLA finds similarly low consistency losses as HOLA, though there HOLA's are lower in the non-quadratic games. Above the threshold, COLA finds consistent updates, even when HOLA does not.

% IPD is a bit of an outlier, consistency-loss wise
For the IPD, COLA's consistency losses are high compared to other games, but much lower than HOLA's consistency losses, especially at high look-ahead rates. We leave it to future work to find methods that obtain more consistent solutions on the IPD. In general, COLA finds consistent updates above the look-ahead threshold even when HOLA does not.

% Do HOLA and COLA find similar update functions?
% When HOLA's updates converge, very similar to COLA
% When diverge, not similar
Third, we are interested whether COLA and HOLA find similar solutions, especially when the consistency losses differ. We calculate the cosine similarity between the respective update functions over $\Theta$. As we can see in Table \ref{tab:tandem_cos}, \ref{tab:imp_sim} and \ref{tab:ipdsim}, COLA and HOLA find very similar solutions when HOLA's updates converge, i.e., when the look-ahead rate is below the threshold. Above the threshold, COLA's and HOLA's updates unsurprisingly become less similar with increasing order, as HOLA's updates diverge with increasing order.
